Neural Mean Discrepancy for Efficient Out-of-Distribution Detection

Various approaches have been proposed for out-of-distribution (OOD) detection by augmenting models, input examples, training sets, and optimization objectives. Deviating from existing work, we have a simple hypothesis that standard off-the-shelf models may already contain sufficient information about the training set distribution which can be leveraged for reliable OOD detection. Our empirical study on validating this hypothesis, which measures the model activation's mean for OOD and in-distribution (ID) mini-batches, surprisingly finds that activation means of OOD mini-batches consistently deviate more from those of the training data. In addition, training data's activation means can be computed offline efficiently or retrieved from batch normalization layers as a 'free lunch'. Based upon this observation, we propose a novel metric called Neural Mean Discrepancy (NMD), which compares neural means of the input examples and training data. Leveraging the simplicity of NMD, we propose an efficient OOD detector that computes neural means by a standard forward pass followed by a lightweight classifier. Extensive experiments show that NMD outperforms state-of-the-art OOD approaches across multiple datasets and model architectures in terms of both detection accuracy and computational cost.

==> cvpr_tables/tab_abla.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
% \begin{tabular}{ccccccc|ccc}
\begin{tabular}{ccc|c}
\toprule
    \begin{tabular}[c]{@{}c@{}} In dist. \end{tabular} &
    \begin{tabular}[c]{@{}c@{}} OOD \end{tabular} &
    \begin{tabular}[c]{@{}c@{}} Method \end{tabular} &
    % \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Train \\ OOD \end{tabular}} &
     {\tiny TNR at TPR 95\% $\uparrow$ / AUROC $\uparrow$ / ACC $\uparrow$ } \\                
\midrule
\multirow{3}{*}{ \begin{tabular}[c]{@{}c@{}} CIFAR-10 \\ (ResNet-34) \end{tabular} } & \multirow{3}{*}{CIFAR-100} & \textbf{NMD} & 81.4 / 95.4 / 88.8\\
&&\textbf{NVD}& 79.2 / 95.3 / 88.4\\
&&\textbf{NMD + NVD}& 82.1 / 95.6 / 89.1\\
\bottomrule
\end{tabular}}
% \vspace{+0.05in}
\caption{\ang{ADD caption.} I will remove this tab and put it in appendix. we have to write conclusion and limitation. but there is no page left. Is it a good idea? Sounds good. You can just mention the numbers somewhere in the text if needed. Pic k one metric. sure. }
\label{tab:abla}
\end{table}




==> cvpr_tables/tab_few_shot.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{
% \begin{tabular}{ccccccc|ccc}
\begin{tabular}{cccccccc}
\toprule
     \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} In-dist \\ (model) \end{tabular}}  &   \multirow{2}{*}{OOD}      &    ODIN~({\color{green}\textbf{w/o}} FT)       & Maha~({\color{green}\textbf{w/o}} FT)  & Gram~({\color{red}\textbf{w/}} FT)  &Energy~({\color{red}\textbf{w/}} FT)  & Ours-LR~({\color{green}\textbf{w/o}} FT) & Ours-MLP~({\color{green}\textbf{w/o}} FT)           \\ 
     \cline{3-8} 
                                &                                & \multicolumn{5}{c}{ TNR at TPR 95\% / AUROC  / Detection acc. }                \\ 
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}} CIFAR-10 \\(ResNet-34) \end{tabular}}
&  iSUN
& \multicolumn{1}{c}{69.8 / 93.7 / 85.9}
& \multicolumn{1}{c}{67.0 / 96.8 / 92.0}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\
&  SVHN
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\
&  Texture
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\
&  LSUN-C
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\
&  ImageNet-C
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\
&  CIFAR-100       
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\

\bottomrule
\end{tabular}
}
\vspace{+0.05in}
\caption{few shot}
\label{tab:few_shot_data}
\end{table*}

==> cvpr_tables/tab_ipmmethod.tex <==
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccc}
\toprule
Method & Failing Loudly & MMD-D & SAMMD \\
\midrule
Minimum Batch Size & 50 & 100 & 20\\
\bottomrule
\end{tabular}
}
% \vspace{+0.05in}
\caption{}
\label{tab:ipm_bsz}
\end{table}




==> cvpr_tables/tab_with_ood_data.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{
% \begin{tabular}{ccccccc|ccc}
\begin{tabular}{cccccccc}
\toprule
     \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} In-dist \\ (model) \end{tabular}}  &   \multirow{2}{*}{OOD}      &    ODIN~({\color{green}\textbf{w/o}} FT)       & OE~({\color{red}\textbf{w/}} FT)  & Maha~({\color{green}\textbf{w/o}} FT)  &Energy~({\color{red}\textbf{w/}} FT)  &  Ours-LR~({\color{green}\textbf{w/o}} FT) & Ours-MLP~({\color{green}\textbf{w/o}} FT)           \\ 
     \cline{3-8} 
                                &                                & \multicolumn{6}{c}{ TNR at TPR 95\% / AUROC  / Detection acc. }                \\ 
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}} CIFAR-10 \\(ResNet-34) \end{tabular}}
&  iSUN
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{\textbf{}} \\
&  SVHN
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\
&  Texture
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{\textbf{}} \\
&  LSUN-C
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{\textbf{}} \\
&  ImageNet-C
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\
&  CIFAR-100       
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{} \\

\bottomrule
\end{tabular}
}
\vspace{+0.05in}
\caption{with ood data results}
\label{tab:with_ood_data}
\end{table*}
